Temporal Concept Dynamics in Diffusion Models via Prompt-Conditioned Interventions

Diffusion models are usually evaluated by their final outputs, gradually denoising random noise into meaningful images. Yet, generation unfolds along a trajectory, and analyzing this dynamic process is crucial for understanding how controllable, reliable, and predictable these models are in terms of their success/failure modes. In this work, we ask the question: when does noise turn into a specific concept (e.g., age) and lock in the denoising trajectory? We propose PCI (Prompt-Conditioned Intervention) to study this question. PCI is a training-free and model-agnostic framework for analyzing concept dynamics through diffusion time. The central idea is the analysis of Concept Insertion Success (CIS), defined as the probability that a concept inserted at a given timestep is preserved and reflected in the final image, offering a way to characterize the temporal dynamics of concept formation. Applied to several state-of-the-art text-to-image diffusion models and a broad taxonomy of concepts, PCI reveals diverse temporal behaviors across diffusion models, in which certain phases of the trajectory are more favorable to specific concepts even within the same concept type. These findings also provide actionable insights for text-driven image editing, highlighting when interventions are most effective without requiring access to model internals or training, and yielding quantitatively stronger edits that achieve a balance of semantic accuracy and content preservation than strong baselines. Code is available at: https://adagorgun.github.io/PCI-Project/

==> figures/fig_bias.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/bias.pdf}
    \caption{Two bias cases: \textbf{(a) Constant Bias:} the CIS remains flat and consistently above the threshold (e.g., female nurse). In this case, regardless of when the prompt-switching intervention is applied, the generated image never changes. \textbf{(b) Temporal bias:} the CIS varies over time but never crosses the threshold, allowing us to identify at which specific timesteps the trajectory is more biased toward a concept (e.g., an old politician). This reveals temporal dynamics of bias. For comparison, (c) shows global, non-temporal bias detection, which does not apply \ours and simply measures the percentage of final generated images associated with a given concept.} 
    \label{fig:bias}
\end{figure}


==> sections/discussion.tex <==
\section{Discussions}
\label{sec:discussions}

==> tables/table_cross_model_summary.tex <==
\begin{table}[t]
\centering
\caption{}
\label{tab:band-summary}
\setlength{\tabcolsep}{4pt}
\small

\resizebox{\linewidth}{!}{%
\begin{tabular}{
  c c
  *{2}{c}
  *{2}{c}
  *{2}{c}
}
\toprule
\multirow{2}{*}{\textbf{Subcategory}} &
\multirow{2}{*}{\textbf{Context}} &
\multicolumn{2}{c}{\textbf{SD\,2.1}} &
\multicolumn{2}{c}{\textbf{SDXL}} &
\multicolumn{2}{c}{\textbf{SD\,3.5}} \\
% \cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}
& &
\(\tau_{50}\) & \(\tau_{70}\) &
\(\tau_{50}\) & \(\tau_{70}\) &
\(\tau_{50}\) & \(\tau_{70}\) \\
\midrule
Time of day & \textemdash
& 0.79 \textbf{$\pm$ 0.05}  & 0.86 \textbf{$\pm$ 0.04}  
& 0.87 \textbf{$\pm$ 0.03}  & 0.90 \textbf{$\pm$ 0.03} 
& 0.98 \textbf{$\pm$ 0.01}  & 0.98 \textbf{$\pm$ 0.00} 
   \\
\midrule
Weather & \textemdash
& 0.62 \textbf{$\pm$ 0.14}  & 0.74 \textbf{$\pm$ 0.13} 
& 0.63 \textbf{$\pm$ 0.14}  & 0.75 \textbf{$\pm$ 0.13} 
& 0.83 \textbf{$\pm$ 0.04}  & 0.89 \textbf{$\pm$ 0.03} 
   \\
\midrule
Season & \textemdash
& 0.55 \textbf{$\pm$ 0.12}  & 0.68 \textbf{$\pm$ 0.11}
& 0.50 \textbf{$\pm$ 0.14}  & 0.65 \textbf{$\pm$ 0.13}
& 0.85 \textbf{$\pm$ 0.02}  & 0.91 \textbf{$\pm$ 0.03}
   \\
\midrule
Venue & Neutral
& 0.45 \textbf{$\pm$ 0.02}  & 0.53 \textbf{$\pm$ 0.02}
& 0.52 \textbf{$\pm$ 0.03}  & 0.59 \textbf{$\pm$ 0.03}
& 0.80 \textbf{$\pm$ 0.04}  & 0.86 \textbf{$\pm$ 0.03}
   \\
Venue & Action
& 0.83 \textbf{$\pm$ 0.06}  & 0.89 \textbf{$\pm$ 0.07}
& 0.78 \textbf{$\pm$ 0.03}  & 0.85 \textbf{$\pm$ 0.03}
& 0.95 \textbf{$\pm$ 0.01}  & 0.97 \textbf{$\pm$ 0.01}
   \\
\midrule
Style & \textemdash
& 0.62 \textbf{$\pm$ 0.05}  & 0.80 \textbf{$\pm$ 0.07}
& 0.63 \textbf{$\pm$ 0.10}  & 0.75 \textbf{$\pm$ 0.10} 
& 0.91 \textbf{$\pm$ 0.03}  & 0.94 \textbf{$\pm$ 0.02}
\\
\midrule
Actions & \textemdash
& 0.70 \textbf{$\pm$ 0.05}  & 0.85 \textbf{$\pm$ 0.07} 
& 0.71 \textbf{$\pm$ 0.08}  & 0.81 \textbf{$\pm$ 0.08}
& 0.86 \textbf{$\pm$ 0.05}  & 0.91 \textbf{$\pm$ 0.04} 
 \\
\midrule
Gender & \textemdash
& 0.49 \textbf{$\pm$ 0.06}  & 0.58 \textbf{$\pm$ 0.05} 
& 0.49 \textbf{$\pm$ 0.12}  & 0.60 \textbf{$\pm$ 0.12} 
& 0.86 \textbf{$\pm$ 0.06}  & 0.89 \textbf{$\pm$ 0.04}
\\
\midrule
Ethnicity & \textemdash
& 0.26 \textbf{$\pm$ 0.08}  & 0.45 \textbf{$\pm$ 0.13}
& 0.27 \textbf{$\pm$ 0.15}  & 0.42 \textbf{$\pm$ 0.17}
& 0.63 \textbf{$\pm$ 0.08}  & 0.75 \textbf{$\pm$ 0.08}
\\
\midrule
Age Group & \textemdash
& 0.50 \textbf{$\pm$ 0.16}  & 0.65 \textbf{$\pm$ 0.16}
& 0.43 \textbf{$\pm$ 0.09}  & 0.55 \textbf{$\pm$ 0.07}
& 0.73 \textbf{$\pm$ 0.07}  & 0.81 \textbf{$\pm$ 0.04}
 \\
\midrule
Object Size & \textemdash
& 0.81 \textbf{$\pm$ 0.08}  & 0.89 \textbf{$\pm$ 0.03}
& 0.85 \textbf{$\pm$ 0.07}  & 0.93 \textbf{$\pm$ 0.07}
& 0.98 \textbf{$\pm$ 0.01}  & 0.98 \textbf{$\pm$ 0.00}
  \\
\midrule
Object Material & \textemdash
& 0.85 \textbf{$\pm$ 0.08}  & 0.90 \textbf{$\pm$ 0.03}
& 0.72 \textbf{$\pm$ 0.08}  & 0.84 \textbf{$\pm$ 0.07}
& 0.91 \textbf{$\pm$ 0.04}  & 0.95 \textbf{$\pm$ 0.03}
 \\
\midrule
Object Color & \textemdash
& 0.78 \textbf{$\pm$ 0.09}  & 0.85 \textbf{$\pm$ 0.07}
& 0.65 \textbf{$\pm$ 0.16}  & 0.75 \textbf{$\pm$ 0.13}
& 0.83 \textbf{$\pm$ 0.12}  & 0.89 \textbf{$\pm$ 0.08}
  \\
\midrule
Accessories & Headshot
& 0.46 \textbf{$\pm$ 0.06}  & 0.58 \textbf{$\pm$ 0.08} 
& 0.41 \textbf{$\pm$ 0.03}  & 0.52 \textbf{$\pm$ 0.10}
& 0.53 \textbf{$\pm$ 0.04}  & 0.62 \textbf{$\pm$ 0.03}
  \\
\midrule
Traits & \textemdash
& 0.52 \textbf{$\pm$ 0.12}  & 0.69 \textbf{$\pm$ 0.10}
& 0.42 \textbf{$\pm$ 0.09}  & 0.58 \textbf{$\pm$ 0.06}
& 0.69 \textbf{$\pm$ 0.06}  & 0.80 \textbf{$\pm$ 0.06}
  \\
\midrule
Clothing & \textemdash
& 0.55 \textbf{$\pm$ 0.14}  & 0.71 \textbf{$\pm$ 0.11}
& 0.46 \textbf{$\pm$ 0.18}  & 0.62 \textbf{$\pm$ 0.15}
& 0.76 \textbf{$\pm$ 0.10}  & 0.84 \textbf{$\pm$ 0.07}
  \\
\midrule
Emotions & \textemdash
& 0.63 \textbf{$\pm$ 0.25}  & \textemdash
& 0.60 \textbf{$\pm$ 0.21}  & 0.72 \textbf{$\pm$ 0.14}
& 0.87 \textbf{$\pm$ 0.08}  & 0.94 \textbf{$\pm$ 0.02}
 \\
\midrule
Handmade Objects & \textemdash
& 0.75 \textbf{$\pm$ 0.07}  & 0.82 \textbf{$\pm$ 0.05}
& 0.68 \textbf{$\pm$ 0.10}  & 0.81 \textbf{$\pm$ 0.08}
& 0.85 \textbf{$\pm$ 0.06}  & 0.89 \textbf{$\pm$ 0.05}
 \\
\midrule
Animals & Indoor
& 0.86 \textbf{$\pm$ 0.00}  & \textemdash
& 0.53 \textbf{$\pm$ 0.00}  & 0.76 \textbf{$\pm$ 0.00} 
& 0.65 \textbf{$\pm$ 0.00}  & 0.71 \textbf{$\pm$ 0.00} 
 \\
\midrule
Animals & Outdoor
& 0.27 \textbf{$\pm$ 0.10}  & 0.37 \textbf{$\pm$ 0.16}
& 0.46 \textbf{$\pm$ 0.16}  & 0.62 \textbf{$\pm$ 0.22}
& 0.57 \textbf{$\pm$ 0.07}  & 0.63 \textbf{$\pm$ 0.07}
\\
\midrule
Nature Objects & Landscape
& 0.40 \textbf{$\pm$ 0.14}  & 0.57 \textbf{$\pm$ 0.21}
& 0.30 \textbf{$\pm$ 0.12}  & 0.44 \textbf{$\pm$ 0.18}
& 0.72 \textbf{$\pm$ 0.09}  & 0.77 \textbf{$\pm$ 0.09}
 \\
\midrule
Nature Objects & City Sideroad
& 0.76 \textbf{$\pm$ 0.10}  & 0.84 \textbf{$\pm$ 0.11}
& 0.67 \textbf{$\pm$ 0.09}  & 0.82 \textbf{$\pm$ 0.04}
& 0.83 \textbf{$\pm$ 0.03}  & 0.91 \textbf{$\pm$ 0.04}
 \\
% --- add more rows here, each with 12 numbers total (4 per model) ---
\bottomrule
\end{tabular}%
}

\end{table}
